AngleSizer: Enhancing Spatial Scale Perception for the Visually Impaired with an Interactive Smartphone Assistant

Spatial perception, particularly at small and medium scales, is an essential human sense but poses a significant challenge for the blind and visually impaired (BVI). Traditional learning methods for BVI individuals are often constrained by the limited availability of suitable learning environments and high associated costs. To tackle these barriers, we conducted comprehensive studies to delve into the real-world challenges faced by the BVI community. We have identified several key factors hindering their spatial perception, including the high social cost of seeking assistance, inefficient methods of information intake, cognitive and behavioral disconnects, and a lack of opportunities for hands-on exploration. As a result, we developed AngleSizer, an innovative teaching assistant that leverages smartphone technology. AngleSizer is designed to enable BVI individuals to use natural interaction gestures to try, feel, understand, and learn about sizes and angles effectively. This tool incorporates dual vibration-audio feedback, carefully crafted teaching processes, and specialized learning modules to enhance the learning experience. Extensive user experiments validated its efficacy and applicability with diverse abilities and visual conditions. Ultimately, our research not only expands the understanding of BVI behavioral patterns but also greatly improves their spatial perception capabilities, in a way that is both cost-effective and allows for independent learning.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> old-study-result.tex <==
\section{USER STUDY} \label{Cap:User study1}

To evaluate AngleSizer's instructional efficacy of AngleSizer, we devised 20 tasks corresponding to 5 interaction gestures. These tasks served as quantitative measures to evaluate the medium and small-scale spatial perception abilities of the BVI. We omitted a baseline control group  {since} the pre-research user performance served as the initial state without AngleSizer intervention. Another reason is that practical constraints outlined in sections 2.1 and 3 make it impractical for users to undertake 20 tasks in their daily lives involving various-sized rulers and teaching aids.



\subsection{Participants} \label{Cap:5.1 Participants}
 Our study involved 11 participants (7 males and 4 females,  mean age = 32.182, SD = 7.791, Table \ref{tab4:Demographic 14}) who engaged in a 13-day user experiment. {Among them, }5  are totally blind; 3  have blindness with light perception; the left 3 have low vision. Participants received compensation of \$150 upon completing the experiment.


% In order to test the teaching effect of AngleSizer, we set 20 tasks (Table \ref{tab5:Learning Task}) from small to large in accordance with 5 interaction gestures (Section \ref{Cap:4.1 Interaction Gestures}, Figure \ref{Fig3:Five interaction gestures}), as the quantitative task to evaluate the user's medium and small scale ability. We recruited 14 BVI people (9 males and 5 females, mean age = 31.357, SD = 7.438, Table \ref{tab4:Demographic 14}) A 10-day user experiment was conducted. After the whole experiment, participants received \$150 to as compensation. 

%%%%%图表4开始-下调

% 精简表
\begin{table*}  [h]
\footnotesize
\caption{Demographic information of 11 participants of the user study. All information was self-reported}  \label{tab4:Demographic 14}
 \setlength{\tabcolsep}{6pt}{
  \begin{tabular}{cccllcc}
    \toprule
    \textbf{No.} & \textbf{Age} & \textbf{Gender} & \textbf{\makecell{Visual Condition}} & \textbf{\makecell{Phone Model}} & \textbf{\makecell{Educational\\Background}} & \textbf{\makecell{Residential\\Status}}\\
    \midrule
    \ P1 & 24 & M & blind & Honor Nova 6 & bachelor's & with roommates \\
    \ P2 & 27 & M & blind with light perception & Mi 10 Pro & bachelor's & with roommates \\
    \ P3 & 28 & M & blind & Huawei Mate 40 Pro & bachelor's & with wife \\
    \ P4 & 38 & F & low vision & Mi 6 & bachelor's & with husband \\
    \ P5 & 50 & M & low vision & Huawei P9 & bachelor's & with wife \\
    \ P6 & 43 & F & blind & Redmi Note 9 & bachelor's & alone  \\
    \ P7 & 25 & F & low vision & Mi 11 & bachelor's & with family \\
    \ P8 & 32 & M & blind & Redmi Note 8 & bachelor's & with girlfriend \\
    \ P9 & 28 & M &blind with light perception & Mi 10s & bachelor's & with colleagues \\
    \ P10 & 31 & M & blind with light perception & Redmi K30 & bachelor's & with colleagues \\
    \ P11 & 28 & F & blind & Mi 6 & bachelor's & with colleagues \\
  \bottomrule
\end{tabular}}
\end{table*}
%%%%%图表结束

% 原始表
% \begin{table*}  
% \footnotesize
% \caption{Demographic information of 14 participants of user study. All information was self-reported}  \label{tab4:Demographic 14}
%  \setlength{\tabcolsep}{6pt}{
%   \begin{tabular}{cccllcc}
%     \toprule
%     \textbf{No.} & \textbf{Age} & \textbf{Gender} & \textbf{\makecell{Visual Condition}} & \textbf{\makecell{Phone Model}} & \textbf{\makecell{Educational\\Background}} & \textbf{\makecell{Residential\\Status}}\\
%     \midrule
%     \ P1 & 24 & M & blind & Honor Nova 6 & bachelor's & with roommates \\
%     \ P2 & 25 & M & low vision & Honor 20 Pro & bachelor's & with roommates \\
%     \ P3 & 30 & M & blind with light perception & Mi 8 lite & bachelor's & alone \\
%     \ P4 & 27 & M & blind with light perception & Mi 10 Pro & bachelor's & with roommates \\
%     \ P5 & 30 & F & blind with light perception & Mi 11 & master's & with friends \\
%     \ P6 & 28 & M & blind & Huawei Mate 40 Pro & bachelor's & with wife \\
%     \ P7 & 38 & F & low vision & Mi 6 & bachelor's & with husband \\
%     \ P8 & 50 & M & low vision & Huawei P9 & bachelor's & with wife \\
%     \ P9 & 43 & F & blind & Redmi Note 9 & bachelor's & alone  \\
%     \ P10 & 25 & F & low vision & Mi 11 & bachelor's & with family \\
%     \ P11 & 32 & M & blind & Redmi Note 8 & bachelor's & with girlfriend \\
%     \ P12 & 28 & M &blind with light perception & Mi 10s & bachelor's & with colleagues \\
%     \ P13 & 31 & M & blind with light perception & Redmi K30 & bachelor's & with colleagues \\
%     \ P14 & 28 & F & blind & Mi 6 & bachelor's & with colleagues \\
%   \bottomrule
% \end{tabular}}
% \end{table*}
% %%%%%图表结束
\subsection{Task Design} \label{Cap:5.2 Design and Procedure}


In out preliminary research, especially in practical tasks during the DTD, we observed a noticeable correlation between participants' performances in scale-related tasks and their prior training or conscious experience in real-life scenarios. However, this correlation did not imply that tasks can be labeled as ``difficult'' or ``easy''. Considering this, we devised 20 tasks within the range of sizes they are used to on a daily basis encompassing various interaction gestures, as outlined in Table \ref{tab5:Learning Task}.

%%%%%图表5开始-下调
\begin{table}  [h]
  \caption{Learning tasks of different gestures.}  \label{tab5:Learning Task}
 \setlength{\tabcolsep}{3.8mm}{
  \begin{tabular}{lllll}
    \toprule
    \textbf{Gestures} & \textbf{Task} &    &    &    \\
    \midrule
    \textbf{One Finger} & 1cm & 2cm & 4cm & 8cm \\
    \textbf{Two Fingers} & 3cm & 5cm & 6cm & 7cm \\
    \textbf{One Hand} & 25cm & 35cm & 70cm & 100cm \\
    \textbf{Two Hands} & 45cm & 65cm & 85cm & 100cm \\
    \textbf{Body Rotation} & 30° & 45° & 60° & 120° \\
  \bottomrule
\end{tabular}}
\end{table}
%%%%%图表结束


\begin{figure*}[ht] 
  \centering
  \includegraphics[width=\textwidth]{experiment.pdf}
  \caption{A participant is using AngleSizer. (a) Using the one-finger gesture, with the right hand's index finger moving on the screen. (b) Using the two-finger gesture, to measure the distance between the right hand's index and middle fingers on the screen. (c) Using the one-hand gesture, to measure the distance moved by the left hand holding the phone. (d) Using the two-hand gesture. (e) Using the body-rotation gesture, holding the phone parallel to the ground and rotating by an angle.} \label{Fig: Experiment}
  \Description{Process flow of the system at each frame, including getting raw data, checking validity, computing, checking stability, and giving feedback.}
\end{figure*}


\subsection{Design and Procedure} \label{Cap:5.2 Design and Procedure} 




The experimental design consists of four distinct phases{: the first phase (Stage 0), the second and third phases (Stage 1) and the fourth phase (Stage 2)}. {Throughout the experiment, we maintained online communication with participants, offer assistance whenever challenges arose, and kept observing their situation through the backend.}

1) On the 1st day, we installed Anglesizer face-to-face on each participant's personal smartphone. Following installation, a 20-minute instructional session familiarized participants with its usage {(Figure \ref{Fig: Experiment})}, and a test (Stage 0) was conducted in the set test module to acquire their initial spatial perception abilities. 

{2) }Stage1 contains days 2 through 12. The first part is from the 2nd to the 9th day, participants seamlessly integrated learning experiences into their daily routines. They had the flexibility to freely switch among three learning modules and were encouraged to discover study contents while exploring their surroundings. The required study time is about 40 minutes per day, aiming for maximum accuracy in task learning. Additionally, participants tested their learning efforts through self test at the beginning and end of each day.

3) The second part of stage1 is from the 10th to the 12th day, participants would no longer do daily learning but only complete the overall test of 20 tasks twice a day in {the} self test {module}. 

{4) On the last day of the experiment, participants did the 20 tasks for three consecutive rounds in the self test module, and the average value was calculated to represent the spatial perception ability level after learning (Stage 2).}


{Additionally, before and after the experiment, we conducted interviews and administered questionnaires related to participants' spatial perceptions to explore the transformative impact of AngleSizer on their daily lives. The data collection and analysis methods were consistent with the pre-survey (Section \ref{Cap:Preliminary research}).}

%0915









\section{Result} \label{Cap:User study}


To ensure a comprehensive analysis across various tasks, we employ \textit{relative error} ($ \frac{\|operation\ result - task\ value\|}{\|task\ value\|}$) as a metric to gauge the accuracy of participants' performance. We assessed AngleSizer's teaching efficacy among the BVI community through the following three focal points: 1) we evaluated users' overall learning progression by analyzing the shift in their {\itshape relative error} metrics, providing a quantitative measure of spatial cognition improvement; 2) we delved into the comparison of learning effects among different groups of users and gestures to assess AngleSizer's applicability; 3) and we gathered subjective feedback from users, capturing their personal experiences and perspectives regarding AngleSizer's teaching effects. {We conducted an analysis of AngleSizer's teaching effect in the following three aspects: 1) evaluation of the user's overall learning progress by assessing the change in {\itshape relative error}, 2) Learning effects of different vision conditions; 3) the learning models of typical users. Prior to delving into the specifics, it's essential to establish clear definitions for the {\itshape relative error}: the ratio of the absolute error (the absolute difference between the task value and the actual value) to the task value. In addition, we try to explore the reasons for these changes.}




\begin{figure*}[h] 
  \centering
  \includegraphics[width=\textwidth]{effect-curve.pdf}
  \caption{The left part is the bar plot of mean errors of 20 tasks with error bars before and after 13 days' training. The Right part shows the process of the whole training.}        \label{Fig6:Left part is bar plot}
  \Description{The left bar plot shows the mean error rate and standard deviation of Stage 0 and Stage 2. The right curve plot shows the changes in the mean error rate of all tasks}
\end{figure*}


\begin{figure}[h] 
  \centering
  \includegraphics[width=\textwidth]{general-curves.pdf}
  \caption{Change in the means of 20 tasks' test results over the training process. The All Test line is all the test results covering Stage 0, Stage 1 and Stage 2; the First Test line is the first test result from each day during  Stage 1; the Last Test line is the last test results from each day during  Stage 1.}        \label{Fig: General Curves}
  \Description{XXX}
\end{figure}


%%%%%图表6开始-下调
% \begin{table*}   
%    \renewcommand\arraystretch{1.5}
% %  \setlength{\parindent}{26pt}}p{5mm}
%   \caption{ Error rate and variance of task before learning (Stage 0) and after learning (Stage 2). Standard deviation values are in parentheses.}  \label{tab6:Error1}
%   \footnotesize
%   \setlength{\tabcolsep}{6pt}{
%    \begin{tabular}{llllll}
%      \toprule
%      \textbf{}&\textbf{One Finger} &\textbf{Two Fingers} & \textbf{One Hand} &  \textbf{Two Hands} &  \textbf{Angle} \\
%      \midrule
%      \multirow{4}*{\rotatebox{90}{\textbf{Bias and STD}}} & 1cm\ \quad\ \makecell[l]{S0: 0.353(0.236) \\ S2: 0.154(0.099)\\} & 3cm\ \quad\ \makecell[l]{S0: 0.165(0.097) \\ S2: 0.061(0.039)} & 25cm\ \quad\  \makecell[l]{S0: 0.117(0.073) \\ S2: 0.064(0.039)} & 45cm\ \quad\  \makecell[l]{S0: 0.145(0.137) \\ S2: 0.074(0.045)} & 30°\ \quad\  \makecell[l]{S0: 0.370(0.179) \\ S2: 0.067(0.040)} \\
%      \cdashline{2-6}
%      \textbf{} & 2cm\ \quad\ \makecell[l]{S0: 0.177(0.085) \\ S2: 0.131(0.075)} & 5cm\ \quad\ \makecell[l]{S0: 0.419(0.215) \\ S2: 0.155(0.076)} & 35cm\ \quad\  \makecell[l]{S0: 0.127(0.062) \\ S2: 0.061(0.041)} & 65cm\ \quad\  \makecell[l]{S0: 0.250(0.106) \\ S2: 0.180(0.090)} & 45°\ \quad\  \makecell[l]{S0: 0.224(0.147) \\ S2: 0.102(0.037)}\\
     
%      \textbf{} & 4cm\ \quad\ \makecell[l]{S0: 0.152(0.102) \\ S2: 0.076(0.063)} & 6cm\ \quad\ \makecell[l]{S0: 0.158(0.118) \\ S2: 0.046(0.031)} & 70cm\ \quad\  \makecell[l]{S0: 0.261(0.142) \\ S2: 0.153(0.069)} & 85cm\ \quad\  \makecell[l]{S0: 0.069(0.057) \\ S2: 0.046(0.029)} & 60°\ \quad\  \makecell[l]{S0: 0.192(0.120) \\ S2: 0.066(0.029)}\\
     
%      \textbf{} & 8cm\ \quad\ \makecell[l]{S0: 0.454(0.288) \\ S2: 0.177(0.201)} & 7cm\ \quad\ \makecell[l]{S0: 0.287(0.151) \\ S2: 0.149(0.082)} & 120cm\quad  \makecell[l]{S0: 0.165(0.075) \\ S2: 0.107(0.040)} & 100cm\quad  \makecell[l]{S0: 0.273(0.170) \\ S2: 0.086(0.046)} & 120°\quad \makecell[l]{S0: 0.301(0.149) \\ S2: 0.193(0.164)}\\
%      \hline
%      \textbf{Mean(S0/S2)} & 0.205/0.095 & 0.187/0.061 & 0.333/0.167 & 0.179/0.071 &  0.270/0.135 \\
%      \hline
%      \textbf{Reduction} & 0.536 & 0.675 & 0.499 & 0.604 & 0.500 \\
%      \hline
%      \textbf{T-Value} & 5.103 & 7.414 & 5.287 & 5.550 & 5.688 	 \\
%      \hline
%      \textbf{P-Value} & 2.027E-04 & 5.100E-06 & 1.924E-04 & 9.380E-05 & 7.440E-05	 \\
%    \bottomrule
%  \end{tabular}}
%  \end{table*}

\begin{table*}   
   \renewcommand\arraystretch{1.5}
%  \setlength{\parindent}{26pt}}p{5mm}
  \caption{ Relative error and variance of task before learning (Stage 0) and after learning (Stage 2). Standard deviation values are in parentheses.}  \label{tab6:Error1}
  \footnotesize
  \setlength{\tabcolsep}{2pt}{
   \begin{tabularx}{\textwidth}{lp{6mm}Xp{6mm}Xp{6mm}Xp{6mm}Xp{6mm}X}
     \toprule
     \textbf{}& \multicolumn{2}{c}{\textbf{One Finger}} &\multicolumn{2}{c}{\textbf{Two Fingers}} & \multicolumn{2}{c}{\textbf{One Hand}}&  \multicolumn{2}{c}{\textbf{Two Hands}} &  \multicolumn{2}{c}{\textbf{Angle}} \\
     \midrule
     \multirow{8}*{\rotatebox{90}{\textbf{Bias and STD}}} & \multirow{2}{}{1cm} & S0: 0.387(0.235) 
     & \multirow{2}{}{3cm} & S0: 0.382(0.189) & \multirow{2}{}{25cm} & S0: 0.453(0.292) & \multirow{2}{}{45cm} & S0: 0.276(0.154) & \multirow{2}{}{30°} & S0: 0.443(0.201) \\

      & & S2:0.128(0.067) & & S2: 0.045(0.027) & & S2: 0.241(0.176) & & S2: 0.087(0.056) & & S2: 0.122(0.089) \\
     
     \cdashline{2-11}

      & \multirow{2}{}{2cm} & S0: 0.158(0.073) 
     & \multirow{2}{}{5cm} & S0: 0.166(0.070) & \multirow{2}{}{35cm} & S0: 0.277(0.153) & \multirow{2}{}{65cm} & S0: 0.151(0.084) & \multirow{2}{}{45°} & S0: 0.279(0.148) \\

     & & S2:0.081(0.044) & & S2: 0.036(0.023) & & S2: 0.172(0.132) & & S2: 0.063(0.032) & & S2: 0.068(0.050) \\
     
     \cdashline{2-11}

      & \multirow{2}{}{4cm} & S0: 0.136(0.140) 
     & \multirow{2}{}{6cm} & S0: 0.115(0.075) & \multirow{2}{}{70cm} & S0: 0.301(0.142) & \multirow{2}{}{85cm} & S0: 0.126(0.056) & \multirow{2}{}{60°} & S0: 0.208(0.132) \\

     & & S2:0.048(0.019) & & S2: 0.041(0.023) & & S2: 0.082(0.049) & & S2: 0.045(0.026) & & S2: 0.135(0.092) \\

     \cdashline{2-11}

      & \multirow{2}{}{8cm} & S0: 0.169(0.120) 
     & \multirow{2}{}{7cm} & S0: 0.073(0.061) & \multirow{2}{}{120cm} & S0: 0.236(0.105) & \multirow{2}{}{100cm} & S0: 0.155(0.109) & \multirow{2}{}{120°} & S0: 0.189(0.089) \\

     & & S2:0.027(0.026) & & S2: 0.025(0.019) & & S2: 0.078(0.054) & & S2: 0.055(0.040) & & S2: 0.056(0.044) \\
   \bottomrule
 \end{tabularx}}
\end{table*}
 
 \subsection{Evaluation of Teaching Effects.} \label{Cap:5.3.1 The error}


 \subsubsection{{\textbf{Apparent improved accuracy from Stage 0 to Stage 2}}}
 The left bar plot in Figure \ref{Fig6:Left part is bar plot} displays a noticeable reduction in  average relative error and variances across 20 tasks performed by 11 participants before and after training. For individual task evaluation, 20 paired t-tests between Stage 0 and Stage 2 were conducted. Most of the 20 tasks exhibited significant improvement, except {for} One Finger 4cm ($t_{10}$ = -1.8117, $p$ = 0.1001), One Hand 35cm ($t_{10}$ = -1.835, $p$ = 0.0963) and Angle 60° ($t_{10}$ = -1.3699, $p$ = 0.2007) tasks. {To evaluate the general improvement of all tasks, Figure \ref{Fig: General Curves} demonstrates an ideal decreasing trend with initial relative error decreasing from 0.234 to 0.082, representing AngleSizer's excellent teaching effect on all 20 tasks.}

 \subsubsection{{\textbf{Consistent reduction in overall relative error}}}
\replaced{The curves in the right part of Figure \ref{Fig6:Left part is bar plot} demonstrate decline trends in average relative error across 20 tasks throughout three stages. Moreover, Figure \ref{Fig: General Curves} highlights a noticeable decreasing trend in average relative error of all 20 tasks during Stage 1.
It is shown that the overall trend of the ``All Test'' line doesn't strictly exhibit a declining pattern due to the fluctuations among the first tests in a day and the last test one day before. In most cases, the relative error of one day's last test is lower than that of first test in the same day, which illustrates the immediate training effect. On the contrary, the relative error of one day's first test is usually higher than that of last test one day before, which implicates the weaken learning effect without training during the night. However,  the ``First Test'' and ``Last Test'' lines show less fluctuation and the ``All Test'' line presents a general decreasing trend over Stage 1, which proves the sustainable learning effect and that the learning effect overcomes the forgetting effect. These observations underscore AngleSizer's effectiveness in enhancing learning outcomes and promoting sustained progress in spatial awareness, particularly evident during Stage 1.}{As Figure \ref{Fig: General Curves} displayed, the relative error of the first test in a day is usually higher than it of the last test, which proved that there is an improvement effect in the short term. While the trend of the All Test line didn't decrease strictly, the other two lines displayed less fluctuation during the whole Stage 1, which proved AngleSizer's excellent teaching effect and ability to cultivate people's constant spatial awareness.

AngleSizer demonstrably enhances users' precision in practicing size and angle-related tasks. Our research also delved into users' learning processes during the experiment, as depicted in the right half of Figure \ref{Fig6:Left part is bar plot}. The test results are included in the analysis.
}
\subsubsection{{\textbf{Focused improvement in optimal tasks' relative error}}}
{To illustrate AngleSizer's most pronounced impact on participants' spatial perception abilities, we identified tasks where each participant demonstrated the most substantial progress. The corresponding relative error curves for these tasks are depicted in Figure \ref{Fig: Selected Cureves}, complementing the comprehensive performance overview seen in the radar plots of Figure \ref{Fig10: All Radar}.
In contrast to the general decreasing trend observed in overall relative error (Figure \ref{Fig6:Left part is bar plot}), these specifically selected tasks showcased accelerated improvement and reduced fluctuations thereafter. This focused analysis emphasizes AngleSizer's ability to expedite enhancements in spatial perception abilities within specific task domains.}
\deleted{
Analyzing the data from the right side of Figure \ref{Fig6:Left part is bar plot}, we observe that, during the learning process, the relative error for the 20 tasks exhibits fluctuations followed by a gradual stabilization with increased testing instances. Our findings, corroborated by data and user interviews, unveil distinct learning patterns among users during these fluctuations:
1) In the early stage of system intervention, users can quickly adapt to the stable impression stage from breaking the ``wrong'' impression of the original action to approaching the ``correct point'', and the effect can be seen quickly in this process. P11 mentioned that ``Before learning, there is no chance to identify different sizes and angles of fine particles. When asking friends, we cannot get timely and accurate responses. As a result, the period of cognition construction is long and often fuzzy. AngleSizer can accurately respond to different scales in just a few seconds, which improves my learning efficiency and allows me to form impressions very quickly.''
2) There is still a process from ``perception to accurate point of action'' to the formation of ``constant memory''. At this stage, especially with more and more practice tasks, if users neglect to consolidate and distinguish, memory will be blurred again, perceptual confusion will occur, and the error rate will rebound. P4 mentioned that``65cm, 70cm, and 80cm are close, while 3cm and 4cm are similar. It is easy to learn only one task, but I need to try several times to distinguish the mixed ones.''
3) With the increase of exercises, users' body perception becomes more and more sensitive, and they can distinguish the scales close to the values. At this stage, they have found some memory tricks (Section \ref{Cap:5.3.1 The error}). 
 In Figure \ref{Fig6:Left part is bar plot}, the final three data points on the task curve represent the outcomes of direct user assessments conducted over an 8-10 day period during the experiment, without any intervening study sessions. The curve's trend indicates that even when the system is temporarily suspended for corrections, users' abilities remain relatively stable, with no significant signs of forgetting. Consequently, our AngleSizer instructional approach appears to result in consistent improvements in user abilities.
}
{\subsection{{Assessment of Applicability}} \label{Cap: 6.2Assessment of Applicability}}
\subsubsection{{\textbf{General improvement across varied visual impairment groups}}}
{
Figure \ref{Fig: Comparison (a)} demonstrates a consistent decrease in relative error across diverse visual impairment groups following AngleSizer training. Statistical analysis unveils significant enhancements in scale perception abilities for the blind ($t_{4}$ = -10.0870, $p$ = 0.0005), low vision ($t_{2}$ = -5.0809, $p$ = 0.0366), and blind with light perception ($t_{2}$ = -4.1024, $p$ = 0.0546) groups.
While the improvement trend in the blind with light perception group doesn't reach statistical significance ($p$ = 0.0546 > 0.05) based on the two samples t-test, it's noteworthy that the results indicate a significant improvement trend. This suggests the potential for a more substantial effect with larger sample sizes. These findings underscore AngleSizer's widespread effectiveness in fostering and refining scale perception skills among individuals with diverse visual impairments, showcasing its applicability in catering to various user needs.
}
\subsubsection{{\textbf{Versatile improvement across gesture categories}}}
{
The comparative analysis between pre- and post-training data across five distinct gesture categories (Figure \ref{Fig: Comparison (b)}) reveals noteworthy enhancements in accuracy. AngleSizer demonstrates substantial reductions in relative error across multiple categories: {\itshape One Finger} ($t_{10}$ = -4.927, $p$ = 0.0006), {\itshape Two Fingers} ($t_{10}$ = -7.480, $p$ < 0.0001), {\itshape One Hand} ($t_{10}$ = -5.977, $p$ = 0.0001), {\itshape Two Hands} ($t_{10}$ = -4.759, $p$ = 0.0008), and {\itshape Body Rotation} ($t_{10}$ = -5.350, $p$ = 0.0003). These findings underscore the effectiveness of AngleSizer in significantly improving spatial perception abilities across a diverse group of gestures. The statistical significance observed across various gesture categories accentuates AngleSizer's applicability and its potential impact on refining spatial accuracy in a wide range of user interactions.
}
 

 
\begin{figure}[H]
    \centering  %图片全局居中
    \subfigure[different groups of BVI people]{
    \label{Fig: Comparison (a)}
    \includegraphics[width=0.45\textwidth]{different-groups.pdf}}
    \subfigure[different interaction gestures]{
    \label{Fig: Comparison (b)}
    \includegraphics[width=0.45\textwidth]{different-gestures.pdf}}
    \caption{{(a) The shifts in relative error across three distinct BVI groups from Stage 0 to Stage 2. (b) The shifts in relative error across five distinct interaction gesture groups from Stage 0 to Stage 2.}}
    \label{Fig: Comparision}
\end{figure}
 

%Figure \ref{Fig8:Changes of five} shows the changes of their relative error over the experimentation of 20 tasks. Overall, although effects vary, they all improved their abilities and made obvious improvements in tasks they were not good at, such as 1cm of one hand and 45deg of body rotation for P13, 30 deg of body rotation for P6, 3cm of two fingers for P8, and 35cm of one hand for P7. Particularly, in Figure \ref{Fig10:(a)}, P13 (a) who has the best improvements had a comparatively poor base at first, but now he has comparable abilities to others after learning. In an aspect of accuracy, P8 (c) is able to make advances even if he has a good foundation, with accuracy further strengthened during learning. Even the user with the worst performance, P7 (d), can still do accurately, except for some tasks such as 70cm with one hand and 65cm with two hands.

\begin{figure} 
    \centering
    \includegraphics[width=\textwidth]{selected-curves.pdf}
    \caption{participant made the most progress, recording relative errors of all the tests more than only each day's first and last test.} \label{Fig: Selected Cureves}
\end{figure}

\subsection{Subjective Feedback} \label{Cap: 5.4 Subjective Feed}

We adapted the NASA scale to evaluate the user experience of AngleSizer, as outlined in Table \ref{tab7:Participants' reviews}, emphasizing users' positive feedback regarding its usability and efficiency. Figure \ref{Fig: Self Evaluation}, derived from the Rosenberg Self-Esteem Scale (RSE), depicted participants' self-assessment before and after their learning process. Through these questionnaires results and interviews, we conducted comprehensive summaries and gleaned valuable insights into their learning journey.). Timely feedback and corrective guidance is the key to training, which greatly improves the learning efficiency of users. On average, it takes only 192.667 seconds for users to execute the 20 tasks at Stage 2, showing the advantage of efficiency.

\begin{table*}[h]  
\footnotesize
   \renewcommand\arraystretch{1.3}
    \setlength{\tabcolsep}{5.5mm}{
  \caption{Participants' reviews on AngleSizer. 1=Disagree strongly,
5=Agree strongly}  \label{tab7:Participants' reviews}
  \begin{tabular}{lcc}
    \toprule
    \textbf{Opinions} & \textbf{\thead{Average Mark\\ (Max is 5)}} & \textbf{\thead{Standard \\ Deviation}}\\
    \midrule
    The system is helpful for me to know sizes and angles better based on my own parts. & 4.727 & 0.467 \\ 
    It's easy to understand the interaction gestures of AngleSizer. & 4.636 & 0.505\\
    It's easy to understand AngleSizer's modules and plans of teaching. & 4.636 & 0.505\\
    The system's teaching improves my understanding of precise sizes and angles. & 4.455 & 0.522\\
    The system's teaching improves my overall understanding of spatial scales. & 4.545 & 0.522\\
    Real-time feedback improves the efficiency of my studying and exploring sizes and angles. & 4.545 & 0.522\\
    I think it's meaningful to use cell phones to learn about sizes and angles. & 4.455 & 0.522 \\
  \bottomrule
\end{tabular}}
\end{table*}

\subsubsection{{\textbf{Factors contributing to learning progress.}}}
Timely feedback is identified as crucial for training, with users emphasizing AngleSizer's real-time feedback on movement sizes or angles, coupled with flexible gesture switching, leading to a richer and more accurate perception, significantly improving learning efficiency. Participants also shared effective learning methods for different tasks, such as \itshape ``experiencing the feeling of arm soreness'' (P4), \itshape ``feeling the range of motion of hand swing'' (P8), \itshape ``feeling the degree of bending of fingers and arms, and the duration of exercise'' (P1), and \itshape ``comprehensively judging combined with surrounding objects and space'' (P5). Moreover, the cooperation of the three modules has narrowed the gap between cognition and practice, and increased their scale reserves (P1, P3-P8, P11).) shows the changes in users' self-ratings.

\subsubsection{{\textbf{Insights from gesture-based learning experiences.}}}
We also received feedback about Gesture-based learning experiences. Finger-based gestures, reliant on finger joint angles and screen edges as references, are noted to aid comprehension significantly (P8, P11). The {\itshape Two Fingers} gesture offers mutual references, facilitating easier mastery compared to the {\itshape One Finger} gesture (P3). Similar distinctions were observed between the {\itshape One Hand} and {\itshape Two Hand} gestures, utilizing various body parts such as eyes, neck, chest, and legs as additional points of reference (P8, P9). Muscle soreness in the arms contributed significantly to the learning process (P2).Exploring angle learning through body rotation extends previous limited plane perception and enhances the body's clarity in perceiving turning and the original position (P5). Furthermore, participants expressed heightened expectations for system capabilities. For instance, P2 suggested enhanced precision in feedback mechanisms, proposing auditory cues like changing frequencies alongside vibrations for more accurate corrections near the target.

\subsubsection{{\textbf{Preference for learning modules.}}}



\subsubsection{{\textbf{Positive impact on participants' lives.}}}
The self-ratings changes in Figure \ref{Fig: Self Evaluation} echo these positive shifts. Participants also positively acknowledge the meaning of learning sizes and angles (see Table \ref{tab7:Participants' reviews}). They all mentioned the newfound importance of learning scales, noting a marked improvement in understanding scale information. After learning, especially using the free exploration module, their understanding of scale information became accurate, as P10 said, {\itshape``Compared to my imagination, the real 1 cm is much smaller, and 85 cm is bigger. Many cognitive biases have been reduced.''}. Their information exchange process is much smoother, as P6 mentioned, {\itshape ``In the dance class, I can accurately understand the teacher's movement guidance on how to turn the body makes my learning experience smoother!''} Most importantly, the improved spatial perception ability helped them solve problems related to size in their daily life, as P9 said, {\itshape``I know how wide the music equipment is in reality trough the parameters when purchasing it online.''}





\begin{figure}[h] 
    \centering
    \includegraphics[width=0.7\textwidth]{self-evaluation.pdf}
    \caption{ Bar plot of 11 users' self-evaluations before and after using AngleSizer on a 5-point Likert scale.}
    \label{Fig: Self Evaluation}
\end{figure}

